Prospects for $B_c^+$ and $B^+\to \tau^+ \nu_\tau$ at FCC-ee

The prospects are presented for precise measurements of the branching ratios of the purely leptonic $B_c^+ \to \tau^+ \nu_\tau$ and $B^+ \to \tau^+ \nu_\tau$ decays at the Future Circular Collider (FCC). This work is focused on the hadronic $\tau^{+} \to \pi^+ \pi^+ \pi^- \bar{\nu}_\tau$ decay in both $B_c^+ \to \tau^+ \nu_\tau$ and $B^+ \to \tau^+ \nu_\tau$ processes. Events are selected with two Boosted Decision Tree algorithms to optimise the separation between the two signal processes as well as the generic hadronic $Z$ decay backgrounds. The range of the expected precision for both signals are evaluated in different scenarios of non-ideal background modelling. This paper demonstrates, for the first time, that the $B^+ \to \tau^+ \nu_\tau$ decay can be well separated from both $B_c^+ \to \tau^+ \nu_\tau$ and generic $Z\to b\bar{b}$ processes in the FCC-ee collision environment and proposes the corresponding branching ratio measurement as a novel way to determine the CKM matrix element $|V_{ub}|$. The theoretical impacts of both $B^+ \to \tau^+ \nu_\tau$ and $B_c^+ \to \tau^+ \nu_\tau$ measurements on New Physics cases are discussed for interpretations in the generic Two-Higgs-doublet model and leptoquark models.

==> experimental-setup.tex <==
\section{Experimental environment}
\label{sec:experimental-setup}



\subsection{FCC-ee}
The international Future Circular Collider (FCC) study aims at a design of $p$-$p$, $\rm e^{+}e^{-}$, and $e$-$p$ colliders to be built in a new 100~km tunnel in the Geneva region. 
The $\rm e^{+}e^{-}$ collider (FCC-ee) has a centre of mass energy range between 91 (\Z-pole) and 375~GeV ($t\bar{t}$). The FCC-ee offers unprecedented possibilities for measuring the properties of the four heaviest particles of the SM (the Higgs, \Z, and \W bosons, and the top quark), but also those of the \bquark and \cquark quarks and of the $\tau$ lepton. In addition, circular colliders have the advantage of delivering collisions to multiple interaction regions, which allow different detector designs to be studied and optimised -- up to four are under consideration for FCC-ee. Moreover, the huge statistics anticipated at the \Z{} peak (the so-called ``Tera-\Z{}" run) brings specific challenges, as the systematic uncertainties of the measurements should be commensurate with their small statistical uncertainties. 


\subsection{Simulation of the detector response}
The detector response has been simulated via the \delphes{}~software package~\cite{deFavereau:2013fsa}. It is a C++ framework, performing a fast multipurpose detector response simulation. The simulation includes a tracking system embedded in a magnetic field, calorimeters, and a muon system. The framework is interfaced to standard file formats (e.g.~Les Houches Event File or HepMC) and outputs observables such as reconstructed charged tracks which can be used for dedicated analyses. The simulation of the detector response takes into account the effect of the magnetic field, the granularity of the calorimeters, and sub-detector resolutions. In the pre-release 3.4.3pre10 used for this analysis, \delphes{} provides parameterised track information with the full covariance matrix using the \fasttrack software. % {\color{red}[Ref. to come]}. 

The detector configuration considered is the Innovative Detector for Electron–positron Accelerators (IDEA) concept. It comprises a silicon pixel vertex detector, a large-volume extremely-light short-drift wire chamber surrounded by a layer of silicon micro-strip detectors, a thin, low-mass superconducting solenoid coil, a pre-shower detector, a dual-readout calorimeter, and muon chambers within the magnet return yoke~\cite{Benedikt:2651299}. The \delphes{}~configuration card used for this analysis is accessible in the repository given in Ref.~\cite{helsens_clement_2021_4817845}. Finally, the \kSimDelphes~\cite{valentin_volkl_2021_4748578} project converts \delphes{} objects to \edmhep{}~\cite{valentin_volkl_2021_4785063}, and the subsequent Monte Carlo (MC) production is performed in the common \edmhep{} data format.

\subsection{Monte-Carlo Production}
MC event samples are used to simulate the response of the detector to signal and background processes. Signal and background events are generated with \pythia~\cite{Sjostrand:2014zea} version 8.303 using the leading order cross-section from the generator with no K-factor. Decays of unstable particles are described using \evtgen~\cite{Lange:2001uf} version 02.00.00, in which final-state radiation is generated using \photos~\cite{Davidson:2010ew}. Several important parameters are configured to be the same for all samples in the \pythia steering cards. At FCC-ee~\cite{Benedikt:2651299}, the energy of the beams is distributed according to a Gaussian function. At the \Z{} peak, the beam energy spread amounts to 0.132\% of the incoming beam energy, half the \Z{} boson mass, which equates to 0.0602\,GeV. 
The position of the interaction region depends on the running conditions of the machine. At the \Z{}-pole the bunch length is $\sigma_z = 12.1$\,mm. The bunch dimensions in the transverse plane, at the interaction point (IP), are given by $\sigma_{x,y} = \sqrt{\beta^*_{x,y}\times \epsilon_{x,y}}$, where the values of the $\beta$ function at the IP, and the horizontal and vertical emittance $\epsilon_{x,y}$ are given in the FCC-ee Conceptual Design Report~\cite{Benedikt:2651299}, and result in approximately $\sigma_x=6.4$\,$\mu$m and $\sigma_y=28.3$\,nm. For Gaussian bunches, the PV distribution in $(x, y, z)$ is well approximated by a 3--dimensional Gaussian distribution, with
\begingroup
\allowdisplaybreaks
\begin{align*}
    &\sigma_x^{PV} = 1\bigg{/}\sqrt{2\left(\frac{\mathrm{cos}^2\alpha}{\sigma_x} + \frac{\mathrm{sin}^2\alpha}{\sigma_z}\right)} \simeq \frac{\sigma_x}{\sqrt{2}}\,,\\
    &\sigma_y^{PV} = \frac{\sigma_y}{\sqrt{2}}\,,\\
    &\sigma_z^{PV} =  1\bigg{/}\sqrt{2\left(\frac{\mathrm{cos}^2\alpha}{\sigma_z} + \frac{\mathrm{sin}^2\alpha}{\sigma_x}\right)}\,,
\end{align*}
\endgroup
where $\alpha$ denotes the half-crossing angle of 15\,mrad. This yields values for the primary vertex smearing, $\sigma_x^{PV} = 4.5$\,$\mu$m, $\sigma_y^{PV} = 20$\,nm, and $\sigma_z^{PV} = 0.3$\,mm. 
    
All of the generator configurations and steering cards are documented and preserved~\cite{helsens_clement_2021_4817845}. The production of Monte-Carlo events is achieved using the FCC common tools and CERN computing and storage resources~\cite{helsens_clement_2021_4817856}. Approximately $10^{10}$ events are produced, representing about 55\,TB of disk space. Dedicated productions with orthogonal seeds between the analysis and multivariate training samples have been considered in order to avoid over--training.

\subsection{Analysis framework}
A sophisticated analysis framework has been developed for all FCC analyses using the common \edmhep{} data format. It is based on RDataFrames~\cite{enrico_guiraud_2017_260230}, where C++ code is conveniently compiled in a \textsc{ROOT}~\cite{rene_brun_2019_3895860} dictionary as ``analysers" which are subsequently called in Python~\cite{helsens_clement_2021_4817870}. Several external packages such as \textsc{ACTS}~\cite{xiaocong_ai_2020_3937454}, \textsc{FastJet}~\cite{Cacciari:2011ma}, and \textsc{awkward}~\cite{jim_pivarski_2021_4746371} are included. The analysis code is distributed via the CERN virtual machine file system cvmfs, and can be run locally or on batch systems. The complete software stack used to produce the results in this paper can be accessed and the results reproduced~\cite{key4hep_collaboration_2021_4818082}.

\subsection{Specificity for this analysis}
For this analysis, dedicated new features of the analysis framework have been developed and are explained in this section. 

\textbf{Perfect vertex seeding:}
Excellent vertex finding is crucial for this analysis. While detailed investigations are ongoing to estimate the impact of imperfect vertexing, for the following results it is assumed that vertices can be perfectly seeded. The procedure is to first find all of the MC vertices by selecting stable charged particles originating from the same point. From those MC vertices, reconstruction-level vertices are fitted using the reconstructed tracks associated to the MC particles attached to the MC vertex. A plot comparing the MC and reconstruction-level number of vertices is shown in Fig.~\ref{fig:vertexing} (a). This procedure properly takes into account the migration of higher number of MC tracks to a given reconstructed multiplicity, as illustrated in Fig.~\ref{fig:vertexing} (b), where about 7\% of the three-track reconstructed vertices originate from a four-track MC vertex.


\textbf{Perfect particle identification:}
In the energy range considered for the identification of pions and kaons in the analysis ($\sim10$\,GeV), extremely good discrimination is expected. For this study, it is thus assumed that pions and kaons can be perfectly identified. This perfect identification is based on preliminary studies which must be confirmed in future with real data~\cite{Wilkinson:2021ehf}. 


\begin{figure}[h!]
\centering
\includegraphics[width = 0.49\textwidth]{figs/mc_vs_reco_vertices.pdf} \put(-165,180){(a)}
\includegraphics[width = 0.49\textwidth]{figs/three_track_vertex_eff.pdf}\put(-165,180){(b)}
\caption{(a) Comparison of normalised number of truth-level MC vertices (red) and number of reconstructed vertices (blue), where MC vertices with one or more charged particle are shown. (b) Proportion of three-track reconstructed vertices that correspond to MC vertices with different numbers of charged particles. Over 90\% of reconstructed three-track vertices originate from a true three-track MC vertex.}
\label{fig:vertexing}
\end{figure}


Processing the first stage of the analysis over the full sample statistics, and calculating  complex quantities (such as the thrust described in Section~\ref{subsection:thrust}, vertexing, building the candidates), takes approximately half a day on a batch system. The total sample size after first-stage processing is $\sim280$\,GB, representing a reduction factor of 200. The second stage of the analysis can then be run locally very quickly, as can all of the final analysis steps described in Section~\ref{sec:analysis}. 

==> notes-on-draft.tex <==
\section*{Notes on draft}

\textcolor{red}{
This version of paper draft is frozen on March 13, 2023 for internal reviews.
The paper is complete, except for a few minor points to be updated:
\begin{itemize}
    \item Is the last sentence of Introduction still valid? Is there an official statement regarding FCC organisation?
    \item We need to make a public reference for the updated FCC software repo. Referred at the beginning of Section~\ref{sec:analysis}
    \item There is a recent (preliminary) result from LHCb on the $R(D^*)$. There could be another update from Belle II. Pheno interpretations in this paper will be updated once those results are released, but the changes are very minor with this LHCb result.
\end{itemize}
}

